A Geometric Analysis of Neural Collapse with Unconstrained Features

We provide the first global optimization landscape analysis of $Neural\;Collapse$ -- an intriguing empirical phenomenon that arises in the last-layer classifiers and features of neural networks during the terminal phase of training. As recently reported by Papyan et al., this phenomenon implies that ($i$) the class means and the last-layer classifiers all collapse to the vertices of a Simplex Equiangular Tight Frame (ETF) up to scaling, and ($ii$) cross-example within-class variability of last-layer activations collapses to zero. We study the problem based on a simplified $unconstrained\;feature\;model$, which isolates the topmost layers from the classifier of the neural network. In this context, we show that the classical cross-entropy loss with weight decay has a benign global landscape, in the sense that the only global minimizers are the Simplex ETFs while all other critical points are strict saddles whose Hessian exhibit negative curvature directions. In contrast to existing landscape analysis for deep neural networks which is often disconnected from practice, our analysis of the simplified model not only does it explain what kind of features are learned in the last layer, but it also shows why they can be efficiently optimized in the simplified settings, matching the empirical observations in practical deep network architectures. These findings could have profound implications for optimization, generalization, and robustness of broad interests. For example, our experiments demonstrate that one may set the feature dimension equal to the number of classes and fix the last-layer classifier to be a Simplex ETF for network training, which reduces memory cost by over $20\%$ on ResNet18 without sacrificing the generalization performance.

==> Sections/problem-save-March28.tex <==

\subsection{Basics of Deep Network}
Let us consider a neural network for $K$-class classification (in logits), which
in its simplest form, the neural network can be written as
\begin{align*}
    f(\mb \theta;\mb x) \;=\;  \mb W_L \sigma\paren{ \mb W_{L-1} \cdots \sigma \paren{\mb W_1 \mb x + \mb b_1} + \mb b_{L-1} }  + \mb b_L,
\end{align*}
where $\mb \theta = \Brac{ \mb W_k,\mb b_k }_{k=1}^L$ denotes all the network parameters, and $\sigma(\cdot)$ is some nonlinear activation such as ReLU []. In particular, $\mb \theta_{\mb W} = \Brac{ \mb W_1,\mb W_2,\cdots,\mb W_L }$ and $\mb \theta_{\mb b} = \Brac{ \mb b_1,\mb b_2,\cdots, \mb b_L }$ denote the weights and bias of all the $L$ layers. For simplicity, we assume that all the bias are zero, so that $\mb \theta = \mb \theta_{\mb W} = \Brac{ \mb W_k }_{k=1}^L$. Typically, training a deep network involves solving the following optimization problem
\begin{align*}
    \min_{\mb \theta} \; \sum_{k=1}^K \sum_{i=1}^{n_k} \mc L \paren{ f(\mb \theta;\mb x_{k,i}), \mb y_k } \;+\; \frac{\lambda}{2} \norm{\mb \theta}{2}^2,
\end{align*}
where $\mb y_k \in \bb R^K $ is an one-hot vector with only the $k$th entry equal to unity, and $\lambda>0$ is the penalty for weight decay, and $\mc L(\cdot,\cdot)$ is certain loss function such as the cross entropy:
\begin{align*}
    \mc L_{CE}(\mb z,\mb y_k) \;:=\; - \log \paren{  \frac{ \exp(z_k) }{ \sum_{i=1}^K \exp(z_i) } } 
\end{align*}
or the $\ell_2$-loss (i.e., least squares loss)
\begin{align*}
    \mc L_2(\mb z,\mb y_k) \;:=\; \frac{1}{2} \norm{ \mb z - \mb y_k }{2}^2.
\end{align*}
In this work, we 




\subsection{Layer-Peeled Model}

Consider the following layer-peeled model which serves as a surrogate for training neural networks:
\e
\min_{\mW\in\R^{K\times d},\mH\in\R^{d\times N}} f(\mW,\mH) = \frac{1}{N}\sum_{k=1}^K\sum_{i=1}^n \calL(\mW\vh_{k,i},\vy_k) + \frac{\lambdaW}{2}\|\mW\|_F^2 + \frac{\lambdaH}{2}\|\mH\|_F^2+\frac{\lambdab}{2}\|\vb\|_2^2,
\label{eq:obj}\ee
where $N = Kn$, $\mH = \begin{bmatrix}\vh_{1,1} \cdots \vh_{K,n} \end{bmatrix}$, $\vy_k\in\R^K$ is the one-hot vector with 1 in the $k$-th entry, and $\calL$ is the cross-entropy loss. Denote by $\vw_k$ as the $k$-th row of $\mW$, i.e., $\mW = \begin{bmatrix}\vw_1 & \cdots & \vw_K \end{bmatrix}^\top$.


\begin{thm}[Global minima]
	Assume $d> K$. Any global minimizer $(\mW^\star, \mH^\star)$ of \eqref{eq:obj}  obeys 
	\e
	\vh_{k,i}^\star = \sqrt{\frac{\lambdaW}{n\lambdaH}}\vw_k^\star
	\label{eq:global-minima}\ee
for all $1\le i\le n, 1\le k \le K$, where $\|\vw_1^\star\| = \|\vw_2^\star\| = \cdots = \|\vw_K^\star\|$ and the matrix $\frac{1}{\|\vw_1^\star\|}\mW^{\star\top}$ forms a $K$-simplex ETF. 
\label{thm:global-minima}\end{thm}


\begin{thm}[No spurious local minima and strict saddle property]
	Assume $d> K$. Then \eqref{eq:obj} has no spurious local minimum, i.e., any local minimizer is a global minimum of form \eqref{eq:global-minima}. Moreover, any critical point of \eqref{eq:obj} that is not a local minimum is a strict saddle with negative curvature, i.e., the Hessian at this point has negative eigenvalue.
\label{thm:global-geometry}\end{thm}


As a consequence of \Cref{thm:global-geometry}, many local search algorithms are guaranteed to converge to a global solution of \eqref{eq:global-minima}. In particular, the result in \cite{lee2016gradient} ensures that gradient descent with random initialization, the de facto algorithm used in deep learning, almost surely escapes strict saddles and converges to a second-order stationary point which happens to be a global minimum of form \eqref{eq:global-minima} for problem \eqref{eq:obj}.

\subsection{With bias term}

Consider the following layer-peeled model which serves as a surrogate for training neural networks:
\e
\min_{\mW\in\R^{K\times d},\mH\in\R^{d\times N}, \vb\in\R^K} f(\mW,\mH,\vb) = \frac{1}{N}\sum_{k=1}^K\sum_{i=1}^n \calL(\mW\vh_{k,i} + \vb,\vy_k) + \frac{\lambdaW}{2}\|\mW\|_F^2 + \frac{\lambdaH}{2}\|\mH\|_F^2+\frac{\lambdab}{2}\|\vb\|_2^2,
\label{eq:obj}\ee
where $N = Kn$, $\mH = \begin{bmatrix}\vh_{1,1} \cdots \vh_{K,n} \end{bmatrix}$, $\vy_k\in\R^K$ is the one-hot vector with 1 in the $k$-th entry, and $\calL$ is the cross-entropy loss. Denote by $\vw_k$ as the $k$-th row of $\mW$, i.e., $\mW = \begin{bmatrix}\vw_1 & \cdots & \vw_K \end{bmatrix}^\top$.


\begin{thm}[Global minima]
	Assume $d> K$. Any global minimizer $(\mW^\star, \mH^\star,\vb^\star)$ of \eqref{eq:obj}  obeys $\vb^\star = \vzero$ and
	\e
	\vh_{k,i}^\star = \sqrt{\frac{\lambdaW}{n\lambdaH}}\vw_k^\star
	\label{eq:global-minima}\ee
for all $1\le i\le n, 1\le k \le K$, where $\|\vw_1^\star\| = \|\vw_2^\star\| = \cdots = \|\vw_K^\star\|$ and the matrix $\frac{1}{\|\vw_1^\star\|}\mW^{\star\top}$ forms a $K$-simplex ETF. 
\label{thm:global-minima}\end{thm}


\begin{thm}[No spurious local minima and strict saddle property]
	Assume $d> K$. Then \eqref{eq:obj} has no spurious local minimum, i.e., any local minimizer is a global minimum of form \eqref{eq:global-minima}. Moreover, any critical point of \eqref{eq:obj} that is not a local minimum is a strict saddle with negative curvature, i.e., the Hessian at this point has negative eigenvalue.
\label{thm:global-geometry}\end{thm}


As a consequence of \Cref{thm:global-geometry}, many local search algorithms are guaranteed to converge to a global solution of \eqref{eq:global-minima}. In particular, the result in \cite{lee2016gradient} ensures that gradient descent with random initialization, the de facto algorithm used in deep learning, almost surely escapes strict saddles and converges to a second-order stationary point which happens to be a global minimum of form \eqref{eq:global-minima} for problem \eqref{eq:obj}.
